Robotic self-representation improves manipulation skills and transfer learning

Cognitive science suggests that the self-representation is critical for learning and problem-solving. However, there is a lack of computational methods that relate this claim to cognitively plausible robots and reinforcement learning. In this paper, we bridge this gap by developing a model that learns bidirectional action-effect associations to encode the representations of body schema and the peripersonal space from multisensory information, which is named multimodal BidAL. Through three different robotic experiments, we demonstrate that this approach significantly stabilizes the learning-based problem-solving under noisy conditions and that it improves transfer learning of robotic manipulation skills.

==> 2_RelatedWorks.tex <==
\section{RELATED WORKS}
\label{sec:related}

\textbf{Topic 1: Multisensory representation learning in robotics}
This relates to two main sensorimotor representations, namely body representation\footnote{This representation includes body schema, body image and body description map} and peripersonal space (PPS) representation. 
\TODO{add ref. here}
Body representation serves as a mean for pose estimation of agents' body parts, coordinate transformation between sensory sources and thus enables action~\cite{hoffmann_body_2010,Gallese2010TheAction}. Robotics and computational models for this representation mostly focus on exploiting sensory information from proprioceptive and tactile sensing~\cite{Roncone2014AutomaticRobot, Li2015TowardsSelf-touch, Vicente2016OnlineFeedback, Hoffmann2018RoboticCortex}, or proprioceptive and visual sensing~\cite{Lallee2013Multi-modalImagery, Schillaci2014OnlineModel,Wijesinghe2018RobotIntegration, Nguyen2018TransferringTasks, Lanillos2018AdaptiveCoding}. On the other hand, PPS representation plays as an interface between the agent's body and the environment through multisensory integration, which maps sensory stimuli to agent's movements (both voluntary and involuntary). Robotics and computational models mainly constructs the PPS representation from vision/audio and touch~\cite{magosso_neural_2010,magosso_visuotactile_2010,serino_extending_2015,straka_learning_2017}, from vision and proprioception~\cite{Antonelli2013On-lineRobot,Chinellato2011ImplicitReaching,juett_learning_2018} or including also touch~\cite{Roncone2016PeripersonalSkin,Nguyen2018CompactInteraction,Nguyen_2019_reaching,Pugach2019Brain-inspiredEvents}. However, while the spatial representation by~\cite{roncone_peripersonal_2016,Nguyen2018CompactInteraction,Pugach2019Brain-inspiredEvents} is formed as the safety margin around robots' body parts for the safety reaction, the representation from others like~\cite{Antonelli2013On-lineRobot,Chinellato2011ImplicitReaching,juett_learning_2018,Nguyen_2019_reaching} is optimized for reaching movements. Most of approaches base on the random movements of joints inspired by infants' motor babbling to generate the training data.

\textbf{Topic 2: Forward model learning}
from multisensory input~\cite{Zambelli:2020:10.1016/j.robot.2019.103312,Copete2017MotorLearning,Hwang2020DealingFramework,Lang2018ARobots} robot learning by imitation with forward model; 

forward model or predictive coding plays roles in high-level cognitive functions of artificial agents (i.e. body-ownership or agency) ~\cite{Lanillos2017YieldingContingencies,Hinz2018DriftingRobot,Lanillos2020RobotMirror}

from single sensory input~\cite{Watter2015EmbedImages,Byravan2018SE3-Pose-Nets:Control,Agrawal2016,Park2018LearningImitate,Pathak2017_curiosity_selfprediction}


\textbf{Topic 3: Intrinsic motivation}
\cite{Dilokthanakul2019FeatureLearning} learning from image only, raw pixel of feature; this may work since the agents get full observation from visual modality. For robot interaction scenarios, learning from only vision will not guarantee the success for all cases~\cite{Lee2020MakingTasks}.
\TODO{add ref. here}
\cite{Pathak2017_curiosity_selfprediction} proposes to use prediction error of an additional forward model as intrinsic motivation to drive gaming agents to explore the space. \cite{pathak19disagreement} further extends the idea by using an ensembles of forward functions and exploiting the disagreement among prediction errors in ensemble as the intrinsic motivation to drive the agents' exploration.
\cite{Roder2020} adopts the ideas of the intrinsic motivation from~\cite{Pathak2017_curiosity_selfprediction} but with only proprioceptive input instead of visual input. Authors also weigh and bound the extrinsic and intrinsic rewards in the range of [-1, 0] with a weighting parameter $\beta$ as similar as~\cite{Dilokthanakul2019FeatureLearning}. Both~\cite{Roder2020,Dilokthanakul2019FeatureLearning} propose models with hierarchical architecture of policies.

While inspired by the ICM model~\cite{Pathak2017_curiosity_selfprediction}, our work has some main differences: (i) We employ the multimodal sensory input instead of only visual input for our model; (ii) The intrinsic motivation in our model relates to ability of anticipating action effects; (iii) We aim to solve the reinforcement learning task in a universal manner; and (iv) Our robots' actions are computed from a deterministic policy in continuous space.
